Efficient Approximate Inference with Walsh-Hadamard Variational Inference

Variational inference offers scalable and flexible tools to tackle intractable Bayesian inference of modern statistical models like Bayesian neural networks and Gaussian processes. For largely over-parameterized models, however, the over-regularization property of the variational objective makes the application of variational inference challenging. Inspired by the literature on kernel methods, and in particular on structured approximations of distributions of random matrices, this paper proposes Walsh-Hadamard Variational Inference, which uses Walsh-Hadamard-based factorization strategies to reduce model parameterization, accelerate computations, and increase the expressiveness of the approximate posterior beyond fully factorized ones.

==> figures/1d_covmatrix/cov_matrix.tex <==
% This file was created by matplotlib2tikz v0.6.18.
\usetikzlibrary{spy}
\begin{tikzpicture}[spy using outlines]

    \begin{groupplot}[group style={group size=2 by 1, horizontal sep=5ex}]
        \nextgroupplot[
            height=2cm,
            width=2cm,
            % tick align=outside,
            % tick pos=left,
            title={cov$\{\gvect\}$},
            % x grid style={white!90.0!black},
            % xmajorgrids,
            xmin=0, xmax=4.5,
            % % xtick={-0.5,1.5},
            % % xticklabels={1,32},
            % xticklabels={},
            % y grid style={white!90.0!black},
            % ymajorgrids,
            ymin=0, ymax=4.5,
            % ytick={-0.5,1.5},
            xtick=\empty, ytick=\empty,
            axis lines=none,
            % yticklabels={32,1}
            % yticklabels={},
            % % enlargelimits=false,
            % scale only axis,
            % axis on top
        ]
        \addplot graphics [includegraphics cmd=\pgfimage,xmin=.5, xmax=2, ymin=4.5, ymax=3, ] {figures/1d_covmatrix/cov_matrix-000.png};
        \spy [blue,draw,height=1.35cm,width=1.35cm,magnification=9,connect spies] on (0.116, 0.349) in node at (-.1, -.75);
        \nextgroupplot[
            colorbar,
            colorbar/width=2mm,
            colorbar style={
                    % ytick={0,.125,.25,.375,0.5,.625,0.75,.875,1},
                    % yticklabels={$\mathdefault{-1.00}$,$\mathdefault{-0.75}$,$\mathdefault{-0.50}$,$\mathdefault{-0.25}$,$\mathdefault{0.00}$,$\mathdefault{0.25}$,$\mathdefault{0.50}$,$\mathdefault{0.75}$,$\mathdefault{1.00}$},
                    ytick={0,.25,0.5,0.75,1},
                    yticklabels={$\mathdefault{-1.0}$,$\mathdefault{-0.5}$,$\mathdefault{0.0}$,$\mathdefault{0.5}$,$\mathdefault{1.0}$},
                    ylabel={}},
            colormap={mymap}{[1pt]
                    rgb(0pt)=(0.403921568627451,0,0.12156862745098);
                    rgb(1pt)=(0.698039215686274,0.0941176470588235,0.168627450980392);
                    rgb(2pt)=(0.83921568627451,0.376470588235294,0.301960784313725);
                    rgb(3pt)=(0.956862745098039,0.647058823529412,0.509803921568627);
                    rgb(4pt)=(0.992156862745098,0.858823529411765,0.780392156862745);
                    rgb(5pt)=(0.968627450980392,0.968627450980392,0.968627450980392);
                    rgb(6pt)=(0.819607843137255,0.898039215686275,0.941176470588235);
                    rgb(7pt)=(0.572549019607843,0.772549019607843,0.870588235294118);
                    rgb(8pt)=(0.262745098039216,0.576470588235294,0.764705882352941);
                    rgb(9pt)=(0.129411764705882,0.4,0.674509803921569);
                    rgb(10pt)=(0.0196078431372549,0.188235294117647,0.380392156862745)
                },
            height=3.75cm,
            width=3.75cm,
            % tick align=outside,
            % tick pos=left,
            title={cov$\{\vect(\Wmatr)\}$},
            x grid style={white!90.0!black},
            xmajorgrids,
            xmin=-0.5, xmax=1023.5,
            xtick={-0.5,1023.5},
            xticklabels={},
            % xticklabels={1,1024},
            y grid style={white!90.0!black},
            ymajorgrids,
            ymin=-0.5, ymax=1023.5,
            ytick={-0.5,1023.5},
            % yticklabels={1024,1}
            yticklabels={}
        ]
        \addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=1023.5, ymin=1023.5, ymax=-0.5] {figures/1d_covmatrix/cov_matrix-001.png};
    \end{groupplot}

\end{tikzpicture}

==> figures/gp_wrt_nparameters/legend-fullcov.tex <==
\begin{tikzpicture}
    \definecolor{color2}{rgb}{0.229411764705882,0.570588235294118,0.229411764705882}
    \definecolor{color0}{rgb}{0.194607843137255,0.453431372549019,0.632843137254902}
    \definecolor{color1}{rgb}{0.881862745098039,0.505392156862745,0.173039215686275}

    \pgfplotsset{
        legend image code/.code={
                \draw[mark repeat=2,mark phase=2, line width=5pt]
                plot coordinates {
                        (0cm,0cm)
                        (0.4cm,0cm)        %% default is (0.3cm,0cm)
                        (0.4cm,0cm)         %% default is (0.6cm,0cm)
                    };%
            }
    }

    \begin{axis}[%
            hide axis,
            xmin=1,
            xmax=1,
            ymin=0,
            ymax=0.4,
            legend style={draw=white!15!black,legend cell align=left},
            legend columns=6
        ]

        \addlegendimage{color0}
        \addlegendentry{gp rff - full covariance};
        \addlegendimage{color1}
        \addlegendentry{gp rff - \hvi full covariance};
        \addlegendimage{color2}
        \addlegendentry{sparse gp - full covariance};

    \end{axis}
\end{tikzpicture}


==> figures/gp_wrt_nparameters/legend-fulldiag.tex <==
\begin{tikzpicture}
    \definecolor{color2}{rgb}{0.229411764705882,0.570588235294118,0.229411764705882}
    \definecolor{color0}{rgb}{0.194607843137255,0.453431372549019,0.632843137254902}
    \definecolor{color1}{rgb}{0.881862745098039,0.505392156862745,0.1730392156862750}

    \pgfplotsset{
        legend image code/.code={
                \draw[mark repeat=2,mark phase=2, line width=5pt]
                plot coordinates {
                        (0cm,0cm)
                        (0.4cm,0cm)        %% default is (0.3cm,0cm)
                        (0.4cm,0cm)         %% default is (0.6cm,0cm)
                    };%
            }
    }

    \begin{axis}[%
            hide axis,
            xmin=1,
            xmax=1,
            ymin=0,
            ymax=0.4,
            legend style={draw=white!15!black,legend cell align=left},
            legend columns=6
        ]

        \addlegendimage{color0}
        \addlegendentry{gp rff - mean field};
        \addlegendimage{color1}
        \addlegendentry{gp rff - \hvi};
        \addlegendimage{color2}
        \addlegendentry{sparse gp - mean field};

    \end{axis}
\end{tikzpicture}

